QUILL: Quotation Generation Enhancement of Large Language Models

While Large language models (LLMs) have become excellent writing assistants, they still struggle with quotation generation. This is because they either hallucinate when providing factual quotations or fail to provide quotes that exceed human expectations. To bridge the gap, we systematically study how to evaluate and improve LLMs' performance in quotation generation tasks. We first establish a holistic and automatic evaluation system for quotation generation task, which consists of five criteria each with corresponding automatic metric. To improve the LLMs' quotation generation abilities, we construct a bilingual knowledge base that is broad in scope and rich in dimensions, containing up to 32,022 quotes. Moreover, guided by our critiria, we further design a quotation-specific metric to rerank the retrieved quotations from the knowledge base. Extensive experiments show that our metrics strongly correlate with human preferences. Existing LLMs struggle to generate desired quotes, but our quotation knowledge base and reranking metric help narrow this gap. Our dataset and code are publicly available at https://github.com/GraceXiaoo/QUILL.

==> table.tex <==
\begin{table*}[!htbp]
\centering

\resizebox{\textwidth}{!}{
\begin{tabular}{|c|cc|}
\hline
  \multirow{1}{*}{\textbf{Method}} &
  \multicolumn{1}{c}{\multirow{1}{*}{\textbf{Literal Sentence}}} &
  \multirow{1}{*}
  {\begin{tabular}[c]{|p{5cm}|p{5cm}|p{5cm}}
  \textbf{Recalled List} &
  \textbf{Metric Rerank} &
  \textbf{Human Rerank}
  
  \end{tabular}}
  \\
  \hline
  \multirow{5}{*}{GPT}
  &
  \multirow{5}{*}{\begin{tabular}[c]{@{}p{10cm}@{}}
  \begin{CJK}{UTF8}{gbsn}
康托尔在研究集合论的过程中，深刻认识到数学探索的本质。他认为：{[}Q{]}。这句话强调了在数学研究中，发现和提出新的问题比解决已有问题更为重要。康托尔的集合论突破了传统数学的界限，提出了无穷集合和基数的概念，为数学理论的发展开辟了新的道路。
\end{CJK} \end{tabular}} 
  &
  {\begin{tabular}[c]{|p{5cm}|p{5cm}|p{5cm}}
\begin{CJK}{UTF8}{gbsn} \cellcolor{green5}数学是科学的皇后，而数论是数学的皇后\end{CJK} & \begin{CJK}{UTF8}{gbsn} \cellcolor{green2}新的数学方法和概念，常常比解决数学问题本身更重要\end{CJK} & \begin{CJK}{UTF8}{gbsn} \cellcolor{green1}在数学的领域中，提出问题的艺术比解答问题的艺术更为重要\end{CJK} 
  \\
  \hline
\begin{CJK}{UTF8}{gbsn} \cellcolor{green2}新的数学方法和概念，常常比解决数学问题本身更重要\end{CJK} & \begin{CJK}{UTF8}{gbsn} \cellcolor{green1}在数学的领域中，提出问题的艺术比解答问题的艺术更为重要\end{CJK} & \begin{CJK}{UTF8}{gbsn} \cellcolor{green2}新的数学方法和概念，常常比解决数学问题本身更重要\end{CJK} 
   \\
   \hline
\begin{CJK}{UTF8}{gbsn} \cellcolor{green1}在数学的领域中，提出问题的艺术比解答问题的艺术更为重要\end{CJK} & \begin{CJK}{UTF8}{gbsn} \cellcolor{green3}数学是一种理性的精神，使人类的思维得以运用到最完善的程度\end{CJK} & \begin{CJK}{UTF8}{gbsn} \cellcolor{green3}数学是一种理性的精神，使人类的思维得以运用到最完善的程度\end{CJK}
   \\
    \hline
\begin{CJK}{UTF8}{gbsn} \cellcolor{green3}数学是一种理性的精神，使人类的思维得以运用到最完善的程度\end{CJK} & \begin{CJK}{UTF8}{gbsn} \cellcolor{green4}数学之所以有高声誉，另一个理由就是数学使得自然科学实现定理化，给予自然科学某种程度的可靠性\end{CJK} & \begin{CJK}{UTF8}{gbsn} \cellcolor{green4}数学之所以有高声誉，另一个理由就是数学使得自然科学实现定理化，给予自然科学某种程度的可靠性\end{CJK} 
  \\
  \hline
 \begin{CJK}{UTF8}{gbsn} \cellcolor{green4}数学之所以有高声誉，另一个理由就是数学使得自然科学实现定理化，给予自然科学某种程度的可靠性\end{CJK} & \begin{CJK}{UTF8}{gbsn} \cellcolor{green5}数学是科学的皇后，而数论是数学的皇后\end{CJK} & \begin{CJK}{UTF8}{gbsn} \cellcolor{green5}数学是科学的皇后，而数论是数学的皇后\end{CJK}
  \end{tabular}}
\\
\hline
  \multirow{5}{*}{Ours} &
  \multirow{5}{*}{\begin{tabular}[c]{@{}p{10cm}@{}}
  \begin{CJK}{UTF8}{gbsn}
康托尔在研究集合论的过程中，深刻认识到数学探索的本质。他认为：{[}Q{]}。这句话强调了在数学研究中，发现和提出新的问题比解决已有问题更为重要。康托尔的集合论突破了传统数学的界限，提出了无穷集合和基数的概念，为数学理论的发展开辟了新的道路。
\end{CJK}
  \end{tabular}}
  &
  {\begin{tabular}[c]{|p{5cm}|p{5cm}|p{5cm}}
\begin{CJK}{UTF8}{gbsn} \cellcolor{green5}数学是科学的皇后，而数论是数学的皇后\end{CJK} & \begin{CJK}{UTF8}{gbsn} \cellcolor{green1}礼义以生利，政事以成义\end{CJK} & \begin{CJK}{UTF8}{gbsn} \cellcolor{green1}在数学的领域中，提出问题的艺术比解答问题的艺术更为重要\end{CJK}
  \\
  \hline
\begin{CJK}{UTF8}{gbsn} \cellcolor{green2}新的数学方法和概念，常常比解决数学问题本身更重要\end{CJK} & \begin{CJK}{UTF8}{gbsn} \cellcolor{green5}数学是科学的皇后，而数论是数学的皇后\end{CJK} & \begin{CJK}{UTF8}{gbsn} \cellcolor{green2}新的数学方法和概念，常常比解决数学问题本身更重要\end{CJK}
  \\
  \hline
\begin{CJK}{UTF8}{gbsn} \cellcolor{green1}在数学的领域中，提出问题的艺术比解答问题的艺术更为重要\end{CJK} & \begin{CJK}{UTF8}{gbsn} \cellcolor{green4}数学之所以有高声誉，另一个理由就是数学使得自然科学实现定理化，给予自然科学某种程度的可靠性\end{CJK} & \begin{CJK}{UTF8}{gbsn} \cellcolor{green3}数学是一种理性的精神，使人类的思维得以运用到最完善的程度\end{CJK} 
  \\
  \hline
\begin{CJK}{UTF8}{gbsn} \cellcolor{green3}数学是一种理性的精神，使人类的思维得以运用到最完善的程度\end{CJK} & \begin{CJK}{UTF8}{gbsn} \cellcolor{green3}数学是一种理性的精神，使人类的思维得以运用到最完善的程度\end{CJK} & \begin{CJK}{UTF8}{gbsn} \cellcolor{green4}数学之所以有高声誉，另一个理由就是数学使得自然科学实现定理化，给予自然科学某种程度的可靠性\end{CJK}
  \\
  \hline
\begin{CJK}{UTF8}{gbsn} \cellcolor{green4}数学之所以有高声誉，另一个理由就是数学使得自然科学实现定理化，给予自然科学某种程度的可靠性\end{CJK} & \begin{CJK}{UTF8}{gbsn} \cellcolor{green1}在数学的领域中，提出问题的艺术比解答问题的艺术更为重要\end{CJK} & \begin{CJK}{UTF8}{gbsn} \cellcolor{green5}数学是科学的皇后，而数论是数学的皇后\end{CJK}
\end{tabular}}
\\
\hline
%%%%%%%

  \multirow{5}{*}{UPR}
  &
  \multirow{5}{*}{\begin{tabular}[c]{@{}p{10cm}@{}}
  \begin{CJK}{UTF8}{gbsn}
在荀子的政治哲学中，{[}Q{]}。是一个重要的命题。 礼义不仅是个人行为的规范，也是国家治理的基础。通过礼义，可以实现经济利益的最大化；通过公正的政务，可以实现社会正义。 荀子的这一思想在中国古代政治理论中占有重要地位，对后世的治国理政产生了深远影响。
\end{CJK} \end{tabular}} 
  &
  {\begin{tabular}[c]{|p{5cm}|p{5cm}|p{5cm}}
\begin{CJK}{UTF8}{gbsn} \cellcolor{green3}故不积跬步，无以至千里；不积小流，无以成江海\end{CJK} &
\begin{CJK}{UTF8}{gbsn}\cellcolor{green2}言无常信，行无常贞，惟利所在，无所不倾，若是则可谓小人矣\end{CJK}&
\begin{CJK}{UTF8}{gbsn}\cellcolor{green1}礼义以生利，政事以成义\end{CJK}
  \\
  \hline
\begin{CJK}{UTF8}{gbsn} \cellcolor{green5}倘能生存,我当然仍要学习\end{CJK} & \begin{CJK}{UTF8}{gbsn} \cellcolor{green1}礼义以生利，政事以成义\end{CJK} & \begin{CJK}{UTF8}{gbsn} \cellcolor{green2}言无常信，行无常贞，惟利所在，无所不倾，若是则可谓小人矣\end{CJK}
   \\
   \hline
\begin{CJK}{UTF8}{gbsn} \cellcolor{green4}玉石不经雕琢，就不能成为有用的器物；人如果不学习，就不会明白道理\end{CJK} & 
\begin{CJK}{UTF8}{gbsn} \cellcolor{green4}玉石不经雕琢，就不能成为有用的器物；人如果不学习，就不会明白道理\end{CJK} & 
\begin{CJK}{UTF8}{gbsn} \cellcolor{green3}故不积跬步，无以至千里；不积小流，无以成江海\end{CJK}
   \\
    \hline
\begin{CJK}{UTF8}{gbsn} \cellcolor{green2}言无常信，行无常贞，惟利所在，无所不倾，若是则可谓小人矣\end{CJK} & \begin{CJK}{UTF8}{gbsn} \cellcolor{green3}故不积跬步，无以至千里；不积小流，无以成江海\end{CJK} & \begin{CJK}{UTF8}{gbsn} \cellcolor{green4}玉石不经雕琢，就不能成为有用的器物；人如果不学习，就不会明白道理\end{CJK} \
   \\
  \hline
\begin{CJK}{UTF8}{gbsn} \cellcolor{green1}礼义以生利，政事以成义\end{CJK} & \begin{CJK}{UTF8}{gbsn} \cellcolor{green5}倘能生存,我当然仍要学习\end{CJK} & \begin{CJK}{UTF8}{gbsn} \cellcolor{green5}倘能生存,我当然仍要学习\end{CJK}
  \end{tabular}}
\\
\hline
  \multirow{5}{*}{Ours} &
  \multirow{5}{*}{\begin{tabular}[c]{@{}p{10cm}@{}}
  \begin{CJK}{UTF8}{gbsn}
在荀子的政治哲学中，{[}Q{]}。是一个重要的命题。 礼义不仅是个人行为的规范，也是国家治理的基础。通过礼义，可以实现经济利益的最大化；通过公正的政务，可以实现社会正义。 荀子的这一思想在中国古代政治理论中占有重要地位，对后世的治国理政产生了深远影响。
\end{CJK}
  \end{tabular}}
  &
  {\begin{tabular}[c]{|p{5cm}|p{5cm}|p{5cm}}
\begin{CJK}{UTF8}{gbsn} \cellcolor{green3}故不积跬步，无以至千里；不积小流，无以成江海\end{CJK} & \begin{CJK}{UTF8}{gbsn} \cellcolor{green1}礼义以生利，政事以成义\end{CJK} & \begin{CJK}{UTF8}{gbsn} \cellcolor{green1}礼义以生利，政事以成义\end{CJK}
  \\
  \hline
\begin{CJK}{UTF8}{gbsn} \cellcolor{green3}倘能生存,我当然仍要学习\end{CJK} & \begin{CJK}{UTF8}{gbsn} \cellcolor{green2}言无常信，行无常贞，惟利所在，无所不倾，若是则可谓小人矣\end{CJK} & \begin{CJK}{UTF8}{gbsn} \cellcolor{green2}言无常信，行无常贞，惟利所在，无所不倾，若是则可谓小人矣\end{CJK}
  \\
  \hline
\begin{CJK}{UTF8}{gbsn} \cellcolor{green4}玉石不经雕琢，就不能成为有用的器物；人如果不学习，就不会明白道理\end{CJK} & \begin{CJK}{UTF8}{gbsn} \cellcolor{green4}玉石不经雕琢，就不能成为有用的器物；人如果不学习，就不会明白道理\end{CJK} & \begin{CJK}{UTF8}{gbsn} \cellcolor{green3}故不积跬步，无以至千里；不积小流，无以成江海\end{CJK}
  \\
  \hline
\begin{CJK}{UTF8}{gbsn} \cellcolor{green2}言无常信，行无常贞，惟利所在，无所不倾，若是则可谓小人矣\end{CJK} & \begin{CJK}{UTF8}{gbsn} \cellcolor{green3}故不积跬步，无以至千里；不积小流，无以成江海\end{CJK} & \begin{CJK}{UTF8}{gbsn} \cellcolor{green4}玉石不经雕琢，就不能成为有用的器物；人如果不学习，就不会明白道理\end{CJK}
  \\
  \hline
\begin{CJK}{UTF8}{gbsn} \cellcolor{green1}礼义以生利，政事以成义\end{CJK} & \begin{CJK}{UTF8}{gbsn} \cellcolor{green5}倘能生存,我当然仍要学习\end{CJK} & \begin{CJK}{UTF8}{gbsn} \cellcolor{green5}倘能生存,我当然仍要学习\end{CJK}
\end{tabular}}
\\
\hline

\end{tabular}
}
\caption{ Additional example of recalled candidates reranked via different rerank metrics and human evaluation. 
The indicators [Q] denotes the insertion positions of the given context. A darker shade of green indicates a higher rank bestowed by humans.
}
\label{tab:appendix2}
\end{table*}
